Bootstrapping ADE M-strings

We study elliptic genera of ADE-type M-strings in 6d (2,0) SCFTs from their modularity and explore the relation to topological string partition functions. We find a novel kinematical constraint that elliptic genera should follow, which determines elliptic genera at low base degrees and helps us to conjecture a vanishing bound for the refined Gopakumar-Vafa invariants of related geometries. Using this, we can bootstrap the elliptic genera to arbitrary base degree, including D/E-type theories for which explicit formulas are only partially known. We utilize our results to obtain the 6d Cardy formulas and the superconformal indices for (2,0) theories.

==> GV_data.tex <==
Here we list some GV invariants obtained from the elliptic genera.
\begin{tabular}{c|cccc|}\hline
    $(1,1,1,1,1,1)$ & $2j_+=$0&1&2&3 \\ \hline
     $2j_-=$0& 340 && 182 && 
\end{tabular}
